Logic-Guided Data Augmentation and Regularization for Consistent Question Answering

Many natural language questions require qualitative, quantitative or logical comparisons between two entities or events. This paper addresses the problem of improving the accuracy and consistency of responses to comparison questions by integrating logic rules and neural models. Our method leverages logical and linguistic knowledge to augment labeled training data and then uses a consistency-based regularizer to train the model. Improving the global consistency of predictions, our approach achieves large improvements over previous methods in a variety of question answering (QA) tasks including multiple-choice qualitative reasoning, cause-effect reasoning, and extractive machine reading comprehension. In particular, our method significantly improves the performance of RoBERTa-based models by 1-5% across datasets. We advance the state of the art by around 5-8% on WIQA and QuaRel and reduce consistency violations by 58% on HotpotQA. We further demonstrate that our approach can learn effectively from limited data.

==> sections/acknowledgement.tex <==
This research was supported by ONR N00014-18-1-2826, DARPA N66001-19-2-403, NSF
(IIS1616112, IIS1252835), Allen Distinguished Investigator Award, Sloan Fellowship, and \hanna{add your japan felloswsihp} We thank Antoine Bosselut, Tim Dettmers, Sewon Min, Keisuke Sakaguchi, David Wadden, Yizhong
Wang and the member of UW NLP group and AI2 for their insightful discussions and feedback.

==> sections/task.tex <==
For  globally consistent predictions in question answering, we require responses to follow two important general logical rules: {\it symmetric consistency} and {\it transitive consistency}, which are illustrated in Figure~\Fref{tab:examples_trans_consistency} and are formally described below.

Let $q, p, a$ be a question, a paragraph and an answer predicted by a model. 
$\mathbf{A}$ is a set of answer candidates. 
Each element of $\mathbf{A}$ can be a span in $p$, a class category, or an arbitrary answer choice.
$X = \{q, p, a\}$ represents a logic atom. 

\begin{table*}[t!]
\begin{center}
{\small
\begin{tabular}{c|c|c|c}
\toprule
  & WIQA & QuaRel & HotpotQA \\
  & \citep{Tandon2019WIQAAD} & \citep{tafjord2019quarel} &
  \citep{yang-etal-2018-hotpotqa} \\\hdashline
 reasoning & Causal Reasoning & Qualitative Reasoning & Qualitative Comparison of two entities \\
  format & classification & multiple choice & span extraction \\
\midrule
% & & & Bridge & Comparison \\\hline
\multirow{4}{*}{$p$} &\multirow{4}{*}{\parbox{4.0cm}{The salt water is heated. As the salt water is heated the water becomes a gas. The salt sink to the bottom of the container. }}  & \multirow{4}{*}{\parbox{3.5cm}{Supposed you were standing on the planet Earth and Mercury. When you look up in the sky and see the sun, }}  &  \multirow{4}{*}{\parbox{6.0cm}{{\bf Golf Magazine} is a monthly golf magazine owned by Time Inc. {\bf El Nuevo Cojo Ilustrado} is an American online Spanish language magazine published from Los Angeles, California.}}  \\
&&&\\
&&&\\
&&&\\\hline
\multirow{2}{*}{$q$} &\multirow{2}{*}{\parbox{4.0cm}{If gas condenses to water, is \textcolor{blue}{\bf less} salt being removed from water.}}  & \multirow{2}{*}{\parbox{3.5cm}{Which planet would the sun appear \textcolor{red}{\bf larger}?}}  &  \multirow{2}{*}{\parbox{6.0cm}{El Nuevo Cojo and Golf Magazine, which one is owned by Time Inc?}}  \\
% &&& \\
&&& \\\hline
$\mathbf{A}$ & \{more, less, no effects\} & \{Mercury, Earth\}& \{Golf Magazine, El Nuevo Cojo\}  \\\hline
$a^{*}$ & more  &Mercury & Golf Magazine \\\hline
\multirow{2}{*}{$q_{sym}^{*}$} & \multirow{2}{*}{\parbox{4.2cm}{{If gas condenses to water, is \textcolor{red}{\bf more} salt being removed from water.}}} & \multirow{2}{*}{\parbox{3.5cm}{Which planet would the sun appear \textcolor{blue}{\bf smaller}?}} & \multirow{2}{*}{\parbox{6.0cm}{Golf Magazine El Nuevo Cojo, which one is \hl{\bf not} owned by Time Inc?}}  \\
% &&& \\
&&& \\\hline
$a_{sym}^{*}$ & less & Earth & El Nuevo Cojo\\\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{tab:QA_example} Examples of the augmented data. 
We partially modify context and questions. 
}
\end{table*}


\paragraph{Symmetric consistency}
In a comparison question, small surface variations such as replacing words with their antonyms can reverse the answer, while keeping the overall semantics of the question as before. 
We define symmetry of questions in the context of QA as follows: $(q, p, a^{*})\leftrightarrow (q_{sym}, p, a_{sym}^{*})$, where $q$ and $q_{sym}$ are antonyms of each other, and $a^{*}_{sym}$ is the opposite of the ground-truth answer $a^{*}$ in $\mathbf{A}$.   
For example, the two questions in the first row of \Fref{tab:examples_trans_consistency} are symmetric pairs. 
We define the symmetric consistency of predictions in QA as the following logic rule: 
\vspace{-0.2cm}
\begin{equation}\label{eq:inductive}
\vspace{-0.1cm}
    (q, p, a) \rightarrow (q_{sym}, p, a_{sym}),
\end{equation}
which indicates a system should predict $a_{sym}$ given $(q_{sym}, p)$, if it predicts $a$ for $(q, p)$.



\paragraph{Transitive consistency.}
Transitive inference between three predicates $A,B,C$ is represented as: $A \rightarrow B \wedge B \rightarrow C$ then $A \rightarrow C$ ~\cite{gazes2012cognitive}. 
In the context of QA, the transitive examples are mainly for causal reasoning questions that inquire about the effect $e$ given the cause $c$.
The second row of Figure~\ref{tab:examples_trans_consistency} shows an example where transitive consistency is violated.
\textcolor{red}{Given two questions, $q_1$ and $q_2$, where the effect of $q_1$ ($=e_1$) is equal to the cause of $q_2$($=c_2$), }we define the transitive consistency of predictions as follows:
\vspace{-0.2cm}
\begin{equation}
\vspace{-0.08cm}
    (q_1, p, a_1) \wedge (q_2, p, a_2) \rightarrow (q_{trans}, p, a_{trans}).
\end{equation}
